Online Calibrated and Conformal Prediction Improves Bayesian Optimization

Accurate uncertainty estimates are important in sequential model-based decision-making tasks such as Bayesian optimization. However, these estimates can be imperfect if the data violates assumptions made by the model (e.g., Gaussianity). This paper studies which uncertainties are needed in model-based decision-making and in Bayesian optimization, and argues that uncertainties can benefit from calibration -- i.e., an 80% predictive interval should contain the true outcome 80% of the time. Maintaining calibration, however, can be challenging when the data is non-stationary and depends on our actions. We propose using simple algorithms based on online learning to provably maintain calibration on non-i.i.d. data, and we show how to integrate these algorithms in Bayesian optimization with minimal overhead. Empirically, we find that calibrated Bayesian optimization converges to better optima in fewer steps, and we demonstrate improved performance on standard benchmark functions and hyperparameter optimization tasks.

==> 4c_analysis.tex <==
\section{UNDERSTANDING CALIBRATED BAYESIAN OPTIMIZATION}
% Having provided the formal definition of our algorithm, we can now examine empirically and in more detail how it improves Bayesian optimization.

% \vk{might need to kill section 4, and put a 2x shorter version of 4.1 into section 5}


% We visualize how the confidence interval of the Forrester function evolves with each step for calibrated and plain Bayesian optimization respectively.
% In  Figure~\ref{calibrated-forrestor-epochs} and Figure~\ref{plain-forrestor-epochs}, we can see that the maximum of acquisition function guides the selection of next data point to be evaluated. The uncalibrated method is overconfident about its prediction around the global minimum, due to which the LCB acquisition function does not explore this region. The calibrated method corrects this confidence interval allowing the acquisition function to explore this region. Thus, the global minimum is immediately discovered by the calibrated approach while the plain method gets stuck in the local minimum. 

% This visually shows that the benefits of calibration are apparent whenever the confidence intervals calculated by the base model represent the uncertainties more accurately. 



% \begin{figure}[htb]
% \centering
% \caption{Selected steps of calibrated Bayesian optimization on the Forrester function (green) using the UCB acquisition function (red), starting from the same three initial points as the uncalibrated method. The recalibrator learns after iteration 12 that the model is overconfident, expanding its confidence intervals. This leads the model to explore in $[0.6, 0.9]$ and find the global minimum. Thus, the calibrated method arrives at the global minimum in less number of steps.}
% \label{calibrated-forrestor-epochs}
% \includegraphics[scale=0.25]{figures/calibration_epochs/epoch_4.png}
% \includegraphics[scale=0.25]{figures/calibration_epochs/epoch_9.png}
% \includegraphics[scale=0.25]{figures/calibration_epochs/epoch_11.png}
% \includegraphics[scale=0.25]{figures/calibration_epochs/epoch_14.png}
% \includegraphics[scale=0.25]{figures/calibration_epochs/epoch_17.png}
% \includegraphics[scale=0.25]{figures/calibration_epochs/epoch_19.png}
% % \includegraphics[scale=0.25]{figures/calibration_epochs/epoch_6.png}
% % \includegraphics[scale=0.25]{figures/calibration_epochs/epoch_7.png}
% \end{figure}



==> 6_discussion.tex <==
\section{DISCUSSION}

%\vk{could merge the last 3 sections if running out of space}

\paragraph{Limitations}
% We demonstrate that calibrated Bayesian optimization helps us identify the optima of an objective function in less number of steps on an average, but 
There are still some tasks such as SVHN image classification where calibration does not improve performance. Studying the properties of objective functions where calibrated Bayesian optimization produces lower benefits can be useful in identifying directions for further improvements in the algorithm.

\paragraph{Extensions \& New Applications} Bayesian optimization can use various underlying base models including neural networks (\citep{pmlr-v37-snoek15}), which we have not yet explored.
% It would be interesting to analyse the performance of calibration in a larger variety of underlying models and acquisition functions. 
We would also like to apply our method to novel applications like  Bayesian optimization for discovering chemical structures 
% with desirable properties 
(\citet{G_mez_Bombarelli_2018}). 
%use Bayesian optimization to search within latent space of the Variational Auto-Encoder(VAE) for proposing chemical structures with desirable properties.  
The recalibration dataset is small due to which the design of the calibration algorithm is important. 
%Exploring other calibration methods like distribution calibration (\citep{song2019distribution}) is an important direction for future work. %We have used the idea of calibration for regression given by \citet{kuleshov2018accurate} in this paper. However  %No specific ethical impact of this work was identified at the time of submission. Applications using bayesian optimization should make sure that societal impacts are taken into consideration. 
% Finally, it would be interesting to understand how the performance of our calibration algorithm changes under varying acquisition functions.
% We have used 
% \begin{itemize}
%     \item Can talk about limitations of this method
%     \item Are there any extensions?
%     \item Are there any applications we haven't tried? For example, using Bayesian optimization to search latent space of VAEs...
%     \item You can talk about applying different calibration methods (e.g. distribution calibration from Song et al. or online calibration from Kuleshov and Ermon 2017)
%     \item Please try to come up some ideas yourself, this is an important part of doing research.
% \end{itemize}
